Extensible Datasort Refinements

Refinement types turn typechecking into lightweight verification. The classic form of refinement type is the datasort refinement, in which datasorts identify subclasses of inductive datatypes. Existing type systems for datasort refinements require that all the refinements of a type be specified when the type is declared; multiple refinements of the same type can be obtained only by duplicating type definitions, and consequently, duplicating code. We enrich the traditional notion of a signature, which describes the inhabitants of datasorts, to allow re-refinement via signature extension, without duplicating definitions. Since arbitrary updates to a signature can invalidate the inversion principles used to check case expressions, we develop a definition of signature well-formedness that ensures that extensions maintain existing inversion principles. This definition allows different parts of a program to extend the same signature in different ways, without conflicting with each other. Each part can be type-checked independently, allowing separate compilation.

==> fig-basic-pattern-typing.tex <==

\begin{figure}[htbp]

  \judgbox{\Sigma; \Gamma; p' : A \entails ms : B}{ }
  \begin{mathpar}
     \Infer{}
          {\patjudg{\Sigma; \Gamma}{(p \sect p')}{A}{T}
            \\
            \Sigma; \Gamma; T \entails e : B
            \\
            \Sigma; \Gamma; (p' - p) : A \entails ms : B}
          {\Sigma; \Gamma; p' : A \entails (\Match{p}{e}) \matchor ms : B}
   \end{mathpar}
   
   \judgbox{\Sigma; \Gamma; T \entails e : B}{ }
   ~\\[-24pt]
   \begin{mathpar}
     \Infer{}
          {
          }
          {\Sigma; \Gamma; \emptyset \entails e : B}
     \and
     \Infer{}
          {\Sigma; \Gamma; T \entails e : B
           \\
           \Sigma; \Gamma, \Delta \entails e : B
          }
          {\Sigma; \Gamma; T \union \{\Delta; A\} \entails e : B}
   \end{mathpar}

   \judgbox{\Sigma; \Gamma; p : A \produces T}{ }
   ~\\[-20pt]
   \begin{mathpar}
     \Infer{}
          { }
          {\patjudg{\Sigma; \Gamma}{\emptypattern}{A}{\emptyset}}
     \and
     \Infer{}
          {\patjudg{\Sigma; \Gamma}{\left(\bigsqcup_{c \in \dom{\Sigma}} c~\wildcard\right)}{s}{T}
          }
          {\patjudg{\Sigma; \Gamma}{\wildcard}{s}{T}
          }
     \and
     \Infer{}
          { }
          {\patjudg{\Sigma; \Gamma}{\wildcard}{A}{\{\emptyctx; A\}}
          }
     \and
     \Infer{}
          {\patjudg{\Sigma; \Gamma}{p_1}{A}{T_1}
           \\
           \patjudg{\Sigma; \Gamma}{p_2}{A}{T_2}
          }
          {\patjudg{\Sigma; \Gamma}{p_1 \patunion p_2}{A}{T_1 \union T_2}
          }
     \and
     \Infer{}
          {\patjudg{\Sigma; \Gamma}{p}{A}{\{(\Delta_1; B_1), \dots, (\Delta_n; B_n)\}}}
          {\patjudg{\Sigma; \Gamma}{x \As p}{A}
              {
               \{(\Delta_1, x : B_1; B_1),
                 \dots,
                 (\Delta_n, x : B_n; B_n)\}
              }
          }
     \\
     \Infer{}
         {\patjudg{\Sigma; \Gamma}{p_1}{A_1}{T_1}
          \\
          \patjudg{\Sigma; \Gamma}{p_2}{A_2}{T_2}}
         {\patjudg{\Sigma; \Gamma}{(p_1, p_2)}{A_1 * A_2}{T_1 \crosstrack T_2}}
     \\
     \Infer{}
          {
            t \in \froz{\Sigma}
            \\
            \Sigma \entails s \subsort t
            \\
            \arrayenvbl{
              \text{for all~}(c : C_k) \in \Sigma
              \\
              ~~\cappjudg{\Sigma; \Gamma}{C_k}{p}{t}{T_k}
            }
          }
          {\patjudg{\Sigma; \Gamma}{c(p)}{s}{\bigcup_{k} T_k}}
  \end{mathpar}
%
  \begin{align*}
        \emptyset \crosstrack T  &~=~  \emptyset
    \\
        \big(\{(\Delta; A)\} \union T_1\big) \crosstrack \big\{(\Delta_1; B_1), \dots, (\Delta_n; B_n)\big\}
        &~=~
        \big\{(\Delta, \Delta_1; A * B_1), \dots, (\Delta, \Delta_n; A * B_n)\big\}
        \\
        &~~~\union
        \big(T_1 \crosstrack \{(\Delta_1; B_1), \dots, (\Delta_n; B_n)\}\big)
  \end{align*}

  \judgbox{\cappjudg{\Sigma; \Gamma}{C}{p}{t}{T}}{ }
  ~\\[-1ex]
  \begin{mathpar}
%
%
%
%
%
%
%
%
     \Infer{}
          {\Sigma \entails s \not\subsort t}
          {\cappjudg{\Sigma; \Gamma}{(B \arr s)}{p}{t}{\emptyset}}
     \and
     \Infer{}
          {\Sigma \entails s \subsort t
            \\
            \Sigma; \Gamma; p : B \produces  \{(s_1; B_1), \dots, (s_n; B_n)\}
          }
          {\cappjudg{\Sigma; \Gamma}{(B \arr s)}{p}{t}%
               {
                   \{
                        (\Delta_1; s), \dots, (\Delta_n; s)
                   \}
               }
          }
  \end{mathpar}

  \caption{Typing rules for pattern matching}
  \FLabel{fig:pattern-typing}
\end{figure}



%
%
%


==> fig-refines.tex <==
\begin{figure}[htbp]


  \caption{Unrefined types} %
  \FLabel{fig:refines}
\end{figure}


%
%
%


==> fig-sugar-typing.tex <==
\begin{figure}[htbp]
  \centering

  \judgbox{\Sigma; \Gamma \entails e : A}{ }
  ~\\[-1ex]
  $\vdots$
  ~\textit{(keep all rules from \Figureref{fig:typing})}
  ~\\[-2ex]
  \begin{mathpar}
     \Infer{\TypeDatatype}
          {\dom{\ctors} \sect \dom{\Sigma} = \emptyset
            \\
            \sigjudg{\Sigma, s, \ctors}%
            \\
            \Sigma, s, \ctors, \freeze{s}; \Gamma \entails e : B}
          {\Sigma; \Gamma \entails \datatypedecl{s}{\ctors}{e} : B}
      \\
      \Infer{\TypeRefine}
          {
            \arrayenvbl{
    %
    %
    %
    %
                     \sigjudg{\Sigma, \subsorts, \ctors}
    %
                \\
                \Sigma, \subsorts, \ctors, \freeze{\subsorts}; \Gamma \entails e : B
            }
          }
          {\Sigma; \Gamma
           \entails
           \refinedecl{\subsorts}{\ctors}{e} : B
         }
  \end{mathpar}

  \caption{Typing rules for syntactic sugar}
  \FLabel{fig:sugar-typing}
\end{figure}


%
%
%


==> fig-sugar.tex <==
\begin{figure}[htbp]
  
  \begin{tabular}[t]{l@{}r@{~~~}c@{~~~}l@{}l@{}}
      Expressions   & $e$ & $\bnfas$&
      \multicolumn{2}{l}{\!\!\!\!%
             \dots
       }
       \\ &&&\!\!\!\!\!
              $
              \bnfalt \datatypedecl{s}{\ctors}{e}
              $
%
       \\ &&&\!\!\!\!\!
              $
              \bnfalt \refinedecl{\subsorts}{\ctors}{e}
              $
%
      \\[0.3em]
      Constructor decl.   & $\ctors$ & $\bnfas$&
                  $c : C
                  \bnfalt (c : C \matchor \ctors)$
      \\[0.1em]
      Subsorting decl.   & $\subsorts$ & $\bnfas$&
                  $
                  \cdot
                  \bnfalt
                  s_1 \subsort s_2 ; \subsorts
                  $
  \end{tabular}

  \caption{Syntactic sugar}
  \FLabel{fig:sugar}
\end{figure}


%
%
%

